EvalSVA: Multi-Agent Evaluators for Next-Gen Software Vulnerability Assessment

Software Vulnerability (SV) assessment is a crucial process of determining different aspects of SVs (e.g., attack vectors and scope) for developers to effectively prioritize efforts in vulnerability mitigation. It presents a challenging and laborious process due to the complexity of SVs and the scarcity of labeled data. To mitigate the above challenges, we introduce EvalSVA, a multi-agent evaluators team to autonomously deliberate and evaluate various aspects of SV assessment. Specifically, we propose a multi-agent-based framework to simulate vulnerability assessment strategies in real-world scenarios, which employs multiple Large Language Models (LLMs) into an integrated group to enhance the effectiveness of SV assessment in the limited data. We also design diverse communication strategies to autonomously discuss and assess different aspects of SV. Furthermore, we construct a multi-lingual SV assessment dataset based on the new standard of CVSS, comprising 699, 888, and 1,310 vulnerability-related commits in C++, Python, and Java, respectively. Our experimental results demonstrate that EvalSVA averagely outperforms the 44.12\% accuracy and 43.29\% F1 for SV assessment compared with the previous methods. It shows that EvalSVA offers a human-like process and generates both reason and answer for SV assessment. EvalSVA can also aid human experts in SV assessment, which provides more explanation and details for SV assessment.

==> Algorithm/Algorithm1.tex <==


\begin{algorithm}[!tpb]
    \footnotesize
    \caption{Referencing the preceding one expert}
    \label{algorithm1}
    \begin{algorithmic}[1]
        \REQUIRE Agents Number: $N$, Expert Agents: $E_{1}, E_{2},\cdots, E_{N}$, Communication Rounds: $R$, Chat History List $History$, Vulnerability Assessment Tasks $T_{1}, T_{2},\cdots, T_{8}$
        \ENSURE Results for Vulnerability Assessment Task $Answer$
        \STATE Initialize a vulnerability assessment task $T_i$
        \FOR{$r \leftarrow 0$ to $R$}
            \FOR{$n \leftarrow 0$ to $N$}
                \IF{$History \neq \emptyset$}
                    \STATE $h_{role} \leftarrow E_n$
                    \STATE $h_{answer} \leftarrow E_n(T_i, History)$
                    \STATE $History \leftarrow \{h_{role}, h_{answer}\}$
                \ELSE
                    \STATE $h_{role} \leftarrow E_n$
                    \STATE $h_{answer} \leftarrow E_n(T_i)$
                    \STATE $History \leftarrow \{h_{role}, h_{answer}\}$
                \ENDIF
                \STATE $Answer \leftarrow$ Final $h_{answer}$
            \ENDFOR
        \ENDFOR
        \RETURN $Answer$
    \end{algorithmic}
\end{algorithm}



==> Algorithm/Algorithm2.tex <==
\begin{algorithm}[!tpb]
    \footnotesize
    \caption{Referencing the previous communication}
    \label{algorithm2}
    \begin{algorithmic}[1]
        \REQUIRE Agents Number: $N$, Expert Agents: $E_{1}, E_{2},\cdots, E_{N}$, Communication Rounds: $R$, Chat History List $History$, Vulnerability Assessment Tasks $T_{1}, T_{2},\cdots, T_{8}$
        \ENSURE Results for Vulnerability Assessment Task $Answer$
        \STATE Initialize a vulnerability assessment task $T_i$
        \FOR{$r \leftarrow 0$ to $R$}
            \FOR{$n \leftarrow 0$ to $N$}
                \IF{$History \neq \emptyset$}
                    \STATE $h_{role} \leftarrow E_n$
                    \STATE $h_{answer} \leftarrow E_n(T_i, History)$
                    \STATE $History \leftarrow \{h_{role}, h_{answer}\}$
                \ELSE
                    \STATE $h_{role} \leftarrow E_n$
                    \STATE $h_{answer} \leftarrow E_n(T_i)$
                    \STATE $History \leftarrow History + \{h_{role}, h_{answer}\}$
                \ENDIF
                \STATE $Answer \leftarrow$ Final $h_{answer}$
            \ENDFOR
        \ENDFOR
        \RETURN $Answer$
    \end{algorithmic}
\end{algorithm}

==> Algorithm/Algorithm3.tex <==
\begin{algorithm}[!tpb]
    \footnotesize
    \caption{Simultaneous Assessment}
    \label{algorithm3}
    \begin{algorithmic}[1]
        \REQUIRE Agents Number: $N$, Expert Agents: $E_{1}, E_{2},\cdots, E_{N}$, Communication Rounds: $R$, Chat History List $History$, Vulnerability Assessment Tasks $T_{1}, T_{2},\cdots, T_{8}$
        \ENSURE Results for Vulnerability Assessment Task $Answer$
        \STATE Initialize a vulnerability assessment task $T_i$
        \FOR{$r \leftarrow 0$ to $R$}
            \STATE Initialize current round chat history $History_{c}$
            \FOR{$n \leftarrow 0$ to $N$}
                \IF{$History \neq \emptyset$}
                    \STATE $h_{role} \leftarrow E_n$
                    \STATE $h_{answer} \leftarrow E_n(T_i, History)$
                    \STATE $History_{c} \leftarrow \{h_{role}, h_{answer}\}$
                \ELSE
                    \STATE $h_{role} \leftarrow E_n$
                    \STATE $h_{answer} \leftarrow E_n(T_i)$
                    \STATE $History_{c} \leftarrow \{h_{role}, h_{answer}\}$
                \ENDIF
            \ENDFOR
            \STATE $History \leftarrow History + History_{c}$
            \STATE $Answer \leftarrow$ Final $h_{answer}$
        \ENDFOR
        \RETURN $Answer$
    \end{algorithmic}
\end{algorithm}

==> Algorithm/Algorithm4.tex <==
\begin{algorithm}[!tpb]
    \footnotesize
    \caption{Summarizer Assessment}
    \label{algorithm4}
    \begin{algorithmic}[1]
        \REQUIRE Agents Number: $N$, Expert Agents: $E_{1}, E_{2},\cdots, E_{N-1}$, Summarizer Agent $S$, Communication Rounds: $R$, Chat History List $History$, Vulnerability Assessment Tasks $T_{1}, T_{2},\cdots, T_{8}$
        \ENSURE Results for Vulnerability Assessment Task $Answer$
        \STATE Initialize a vulnerability assessment task $T_i$
        \FOR{$r \leftarrow 0$ to $R$}
            \STATE Initialize current round chat history $History_{c}$
            \FOR{$n \leftarrow 0$ to $N$}
                \IF{$n \neq N$}
                    \STATE $h_{role} \leftarrow E_n$
                    \STATE $h_{answer} \leftarrow E_n(T_i, History)$
                    \STATE $History_{c} \leftarrow \{h_{role}, h_{answer}\}$
                \ELSE
                    \STATE $s_{role} \leftarrow S$
                    \STATE $s_{answer} \leftarrow S(T_i, History + History_{c})$
                    \STATE $History_{c} \leftarrow \{s_{role}, s_{answer}\}$
                \ENDIF
            \ENDFOR
            \STATE $History \leftarrow History + History_{c}$
            \STATE $Answer \leftarrow$ Final $s_{answer}$
        \ENDFOR
        \RETURN $Answer$
    \end{algorithmic}
\end{algorithm}

==> Sections/6_Checklist.tex <==
\newpage
\appendix
\onecolumn

% \section{Limitations}
% \label{limitations}
% \textit{Transferability on Other Types of SV Assessment.} 
% In this paper, we only focus solely on commit-based SV assessment and CVSS v3.1 standard, excluding SV and bug report-based methods. However, \tool can be generalized to all types of SV assessment and other expert-based SV assessment standards because it can be easily updated. In the future, we intend to explore the efficacy of \tool regarding the upgrade of the assessment system.

% \textit{Constraints of Domain Knowledge in Prompts.}
% For the context limited of LLMs, \tool only contains the prompt-based domain knowledge and chat history to facilitate the SV assessment. In the future, we will explore more expert-based examples as prompts for the LLM-based SV assessment.


% \section{Prompt Template}
% \label{template}
% The example of a prompt template is illustrated in Figure~\ref{prompt}. We incorporate numerous commit details, such as commit information, CVE Description, Commit message, and domain knowledge of CVSS. In this context, we substitute the highlighted (red) square brackets with corresponding information from each commit before querying the LLMs.
% \begin{figure*}[t]
% 	\centering
%     \includegraphics[width=0.99\textwidth]{Figures/prompt_cropped.pdf}
% 	\caption{The prompt template for commit-based SV assessment.}
% 	\label{prompt}
% \end{figure*}


% \section{Additional Communication Strategies Results}
% \label{additionalresults}
% In this appendix, we present the detailed experiment results that focus on different communication strategies for Java and C++. Our study is also conducted in ChatGPT as Q2.
% \input{Tables/RQ2_Java_Appendix}
% \input{Tables/RQ2_C++_Appendix}

% % \section{Additional \tool Results}
% \section{Additional Experimental Setting}
% \label{additionalexperimentalsetting}
% \subsection{Implementation Details}

% For ChatGPT (``gpt-3.5-\textit{turbo-0125}'') and GPT-4 (``gpt-4-\textit{turbo}''), we use the public APIs provided by OpenAI. To mitigate the risk of data leakage and effectively evaluate the methods' ability for SV assessment, we adopt a time-split setting based on the ``commit date'' of vulnerability patches.
% Specifically, the vulnerability-related commit after 2023-11-27 of Python, 2023-11-28 of Java, and 2023-12-02 of C++ are designated for testing in this paper.


% \subsection{Additional Metrics}
% We also use the following two widely used performance metrics for SV assessment:

% \textbf{Precision:} It is the ratio of true positives ($\text{TP}$) to the sum of true positives and false positives ($\text{FP}$), calculated following: $\text{Precision} = \frac{\text{TP}}{\text{TP}+\text{FP}}$. 

% \textbf{Recall:} It is the ratio of $\text{TP}$ to the sum of $\text{TP}$ and false negatives ($\text{FN}$), calculated following: $\text{Recall} = \frac{\text{TP}}{\text{TP}+\text{FN}}$. 





% \section{Algorithm of Communication Strategies}
% \label{AlgorithmofCommunication}
% In this appendix, we formally define the following four different communication strategies, including \textit{preceding one expert} (Refer to Algorithm~\ref{algorithm1}), \textit{previous communication}(Refer to Algorithm~\ref{algorithm2}), \textit{simultaneous assessment}(Refer to Algorithm~\ref{algorithm3}), and \textit{summariser assessment}(Refer to Algorithm~\ref{algorithm4}) for the SV assessment task.
% \input{Algorithm/Algorithm1}
% \input{Algorithm/Algorithm2}
% \input{Algorithm/Algorithm3}
% \input{Algorithm/Algorithm4}


% \section{Task-related Prompt}
% \label{taskrelatedprompt}
% In this appendix, we present the task-related prompt by CVSS v3.1 and
% design several descriptions as follows.

% \textbf{Attack Vector}: \textit{You are a [Language] expert for Attack Vector. This metric reflects the context in which vulnerability exploitation is possible. \ This metric value (and consequently the Base Score) will be larger the more remote (logically, and physically) an attacker can be to exploit the vulnerable component. Network (N): The vulnerable component is bound to the network stack and the set of possible attackers extends beyond the other options listed below, up to and including the entire Internet. Local (L): The vulnerable component is not bound to the network stack and the attacker’s path is via read/write/execute capabilities.}

% \textbf{Attack Complexity}: \textit{You are a [Language] expert for Attack Complexity. This metric describes the conditions beyond the attacker’s control that must exist in order to exploit the vulnerability. If a specific configuration is required for an attack to succeed, the Base metrics should be scored assuming the vulnerable component is in that configuration. The Base Score is greatest for the least complex attacks.
% Low (L): Specialized access conditions or extenuating circumstances do not exist. An attacker can expect repeatable success when attacking the vulnerable component.
% High (H): A successful attack depends on conditions beyond the attacker's control. That is, a successful attack cannot be accomplished at will, but requires the attacker to invest in some measurable amount of effort in preparation or execution against the vulnerable component before a successful attack can be expected.}

% \textbf{Privileges Required}: \textit{You are a [Language] expert for Privileges Required. This metric describes the level of privileges an attacker must possess before successfully exploiting the vulnerability. The Base Score is greatest if no privileges are required.
% None (N): The attacker is unauthorized prior to attack, and therefore does not require any access to settings or files of the vulnerable system to carry out an attack.
% Low (L): The attacker requires privileges that provide basic user capabilities that could normally affect only settings and files owned by a user.
% High (H): The attacker requires privileges that provide significant (e.g., administrative) control over the vulnerable component allowing access to component-wide settings and files.}

% \textbf{User Interaction}: \textit{You are a [Language] expert for User Interaction. This metric captures the requirement for a human user, other than the attacker, to participate in the successful compromise of the vulnerable component. This metric determines whether the vulnerability can be exploited solely at the will of the attacker, or whether a separate user (or user-initiated process) must participate in some manner. The Base Score is greatest when no user interaction is required.
% None (N): The vulnerable system can be exploited without interaction from any user.
% Required (R): Successful exploitation of this vulnerability requires a user to take some action before the vulnerability can be exploited.}

% \textbf{Scope}: \textit{You are a [Language] expert for Scope. The Scope metric captures whether a vulnerability in one vulnerable component impacts resources in components beyond its security scope. The Base Score is greatest when a scope change occurs.
% Unchanged (U): An exploited vulnerability can only affect resources managed by the same security authority.
% Changed (C): An exploited vulnerability can affect resources beyond the security scope managed by the security authority of the vulnerable component.}

% \textbf{Confidentiality}: \textit{You are a [Language] expert for Confidentiality. This metric measures the impact to the confidentiality of the information resources managed by a software component due to a successfully exploited vulnerability. The impact can vary from none to complete disclosure of all restricted information to the attacker.
% High (H): There is a total loss of confidentiality, resulting in all resources within the impacted component being divulged to the attacker. Alternatively, access to only some restricted information is obtained, but the disclosed information presents a direct, serious impact.
% Low (L): There is some loss of confidentiality. Access to some restricted information is obtained, but the attacker does not have control over what information is obtained, or the amount or kind of loss is limited.
% None (N): There is no loss of confidentiality within the impacted component.}

% \textbf{Integrity}: \textit{You are a [Language] expert for Integrity. This metric measures the impact to the integrity of a successfully exploited vulnerability. Integrity refers to the trustworthiness and veracity of information. The Base Score is greatest when the consequence to the impacted component is highest.
% High (H): There is a total loss of integrity, or a complete loss of protection. For example, the attacker is able to modify any/all files protected by the impacted component.
% Low (L): Modification of data is possible, but the attacker does not have control over the consequence of a modification, or the amount of modification is limited.
% None (N): There is no loss of integrity within the impacted component.}

% \textbf{Availability}: \textit{You are a [Language] expert for Availability. This metric measures the impact to the availability of the impacted component resulting from a successfully exploited vulnerability. The Base Score is greatest when the consequence to the impacted component is highest.
% High (H): There is a total loss of availability, resulting in the attacker being able to fully deny access to resources in the impacted component; this loss is either sustained (while the attacker continues to deliver the attack) or persistent (the condition persists even after the attack has completed).
% Low (L): Performance is reduced or there are interruptions in resource availability. Even if repeated exploitation of the vulnerability is possible, the attacker does not have the ability to completely deny service to legitimate users.
% None (N): There is no impact to availability within the impacted component.}

\clearpage
\newpage
\begin{center}

\text{} 

\textbf{
\huge
--- Reproducibility Checklist ---
}

\text{} 
% }
\end{center}


Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
    \item Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes)
\end{itemize}

Does this paper make theoretical contributions? (no)

If yes, please complete the list below.

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    \item Proofs of all novel claims are included. (yes/partial/no)
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

Does this paper rely on one or more datasets? (yes)

If yes, please complete the list below.

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
    \item All novel datasets introduced in this paper are included in a data appendix. (yes)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
    \item All datasets that are not publicly available are described in detail, with an explanation why publicly available alternatives are not scientifically satisficing. (yes)
\end{itemize}

Does this paper include computational experiments? (yes)

If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes)
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. (yes)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
    \item This paper states the number of algorithm runs used to compute each reported result. (yes)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)
\end{itemize}

